Strong identifiability and parameter learning in regression with heterogeneous response

Mixtures of regression are a powerful class of models for regression learning with respect to a highly uncertain and heterogeneous response variable of interest. In addition to being a rich predictive model for the response given some covariates, the parameters in this model class provide useful information about the heterogeneity in the data population, which is represented by the conditional distributions for the response given the covariates associated with a number of distinct but latent subpopulations. In this paper, we investigate conditions of strong identifiability, rates of convergence for conditional density and parameter estimation, and the Bayesian posterior contraction behavior arising in finite mixture of regression models, under exact-fitted and over-fitted settings and when the number of components is unknown. This theory is applicable to common choices of link functions and families of conditional distributions employed by practitioners. We provide simulation studies and data illustrations, which shed some light on the parameter learning behavior found in several popular regression mixture models reported in the literature.

==> Macros.tex <==
%\setlength\parindent{0pt}  % no indent

% \setlength{\textwidth}{\paperwidth}
% \addtolength{\textwidth}{-6cm}
% \setlength{\textheight}{\paperheight}
% \addtolength{\textheight}{-4cm}
% \addtolength{\textheight}{-1.1\headheight}
% \addtolength{\textheight}{-\headsep}
% \addtolength{\textheight}{-\footskip}
% \setlength{\oddsidemargin}{0.5cm}
% \setlength{\evensidemargin}{0.5cm}
\usepackage{subcaption}


\usepackage{enumitem}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{epsf}
\usepackage{epsfig}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
% \usepackage{epstopdf}
\usepackage{psfrag}
\usepackage{fullpage}
\usepackage{pdfpages}

\newcommand*{\backrefalt}[4]{%
    \ifcase #1 \footnotesize{(Not cited.)}%
    \or        \footnotesize{(Cited on page~#2.)}%
    \else      \footnotesize{(Cited on pages~#2.)}%
    \fi}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb,bbm}
\usepackage{caption}

\usepackage{algorithm}
\usepackage{algpseudocode}
%\usepackage{algorithmic}
%\usepackage{algorithm}
\usepackage{multicol}
\usepackage{caption}
%\captionsetup[algorithm]{singlelinecheck=off}
\usepackage{color}
%\usepackage{biblatex}
%\addbibresource{refs.bib}
%\bibliographystyle{abbrv}

\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs} % for professional tables
%\usepackage{arxiv}
%\usepackage{enumitem}
\usepackage{url}% for url's in bib
% for theorem hyperlink colors
\usepackage[colorlinks,linkcolor=magenta,citecolor=blue, pagebackref=true,backref=true]{hyperref}
\usepackage{changes}
\usepackage{mathptmx}
\usepackage{anyfontsize}
\usepackage{t1enc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\id}{Id}
\DeclareMathOperator{\cov}{Cov}

\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{observation}{Observation}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}


%\newcommand{\dim}{\textnormal{dim}}

\newenvironment{assumptionprime}[1]
  {\renewcommand{\theassumption}{\ref{#1}$'$}%
   \addtocounter{assumption}{-1}%
   \begin{assumption}}
  {\end{assumption}}

\newcommand{\genecomment}[1]{{\bf{{\blue{{TEAM --- #1}}}}}}
% --- For coloring ---


\renewcommand\arraystretch{1.5}



\newtheorem{innercustomgeneric}{\customgenericname}
\providecommand{\customgenericname}{}
\newcommand{\newcustomtheorem}[2]{%
  \newenvironment{#1}[1]
  {%
   \renewcommand\customgenericname{#2}%
   \renewcommand\theinnercustomgeneric{##1}%
   \innercustomgeneric
  }
  {\endinnercustomgeneric}
}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcustomtheorem{customthm}{Theorem}
\newcustomtheorem{customlemma}{Lemma}
\newcustomtheorem{customprop}{Proposition}

\newcommand{\Ncal}{\mathcal{N}}

\newcommand{\myline}{1.5}
\newcommand{\trace}{\ensuremath{tr}}

\long\def\comment#1{}
\renewcommand\vec[1]{\ensuremath\boldsymbol{#1}}
\newcommand{\Sdd}{\ensuremath{S_{d_2}^{++}}}
\renewcommand{\trace}{\ensuremath{\operatorname{tr}}}
\newcommand{\Ecal}{\ensuremath{\mathcal{E}}}
\newcommand{\Tcal}{\ensuremath{\mathcal{T}}}
\newcommand{\Ocal}{\ensuremath{\mathcal{O}}}
\newcommand{\Gcal}{\ensuremath{\mathcal{G}}}
\newcommand{\Xcal}{\ensuremath{\mathcal{X}}}
\newcommand{\Ycal}{\ensuremath{\mathcal{Y}}}
\newcommand{\Pcal}{\ensuremath{\mathcal{P}}}
\newcommand{\Rbb}{\ensuremath{\mathbb{R}}}
\newcommand{\Pbb}{\ensuremath{\mathbb{P}}}
\newcommand{\underfun}{\ensuremath{G_{0}}}
\newcommand{\mleprob}{\ensuremath{\widehat{G}_{n}}}
\newcommand{\mleweight}{\ensuremath{\widehat{\lambda}_{n}}}
\newcommand{\sureprob}{\ensuremath{\overline{G}_{n}}}
\newcommand{\sureweight}{\ensuremath{\overline{\lambda}_{n}}}
\newcommand{\ambispace}{\ensuremath{\mathcal{G}}}
\newcommand{\overlapset}{\ensuremath{\mathcal{A}}}
\newcommand{\mydefn}{\ensuremath{: =}}
\newcommand{\gaussden}{\ensuremath{f}}
\newcommand{\extraset}{\ensuremath{\mathcal{B}}}
\newcommand{\extraind}{\ensuremath{\mathcal{I}}}
\newcommand{\sumind}{\ensuremath{\mathcal{S}}}
\newcommand{\bigO}{\ensuremath{\mathcal{O}}}
\newcommand{\smallO}{\ensuremath{o}}
\newcommand{\diff}{\ensuremath{\mathcal{T}}}
\newcommand{\distrong}{\ensuremath{\mathcal{D}_{\text{strong}}}}
\newcommand{\disgauss}{\ensuremath{\mathcal{D}_{\text{gauss}}}}

\newcommand{\Poi}{\ensuremath{\text{Poi}}}
\newcommand{\Bin}{\ensuremath{\text{Bin}}}
\newcommand{\NB}{\ensuremath{\text{NB}}}


%\newcommand{\disgaussmod}{\ensuremath{\bar{\mathcal{D}}_{\text{gauss}}}}
\newcommand{\diskew}{\ensuremath{\mathcal{D}_{\text{skew}}}}

%%% Brackets
\newcommand{\brackets}[1]{\left[ #1 \right]}
\newcommand{\parenth}[1]{\left( #1 \right)}
\newcommand{\bigparenth}[1]{\big( #1 \big)}
\newcommand{\biggparenth}[1]{\bigg( #1 \bigg)}
\newcommand{\braces}[1]{\left\{ #1 \right \}}
\newcommand{\abss}[1]{\left| #1 \right |}
\newcommand{\angles}[1]{\left\langle #1 \right \rangle}
\newcommand{\tp}{^\top}

% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\left\| #1\right\|_{#2}}
% \newcommand{\norm}[1]{\vecnorm{#1}{2}} % euclidean norm
\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{fro}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}
\newcommand{\norm}[1]{\left\|#1\right\|}

\newcommand{\dat}[1]{{\bf{{\blue{{Dat - #1}}}}}}
\newcommand{\linh}[1]{{\bf{{\red{{Linh - #1}}}}}}

